The CO-H2 Conversion Factor in Galaxy Mergers

The CO-H2 conversion factor in galaxies is typically described as bimodal: one value for discs and quiescent regions, and another (lower) value for mergers and starbursts. In this proceeding, I will describe both empirical observational evidence that the conversion factor varies with physical environment, as well as a theoretical model which aims to understand the physical processes which drive these variations. I present a functional form for Xco which can be applied to observations ranging in scale from ~70 pc to galaxy-wide scales, and show the consequences of the application of this model to the Kennicutt-Schmidt star formation law.

==> editor/author/aspauthor.tex <==
% This is the aspauthor.tex LaTeX file
% Copyright 2010, Astronomical Society of the Pacific Conference Series

%\documentclass[11pt,twoside]{article}
%\usepackage{./asp2010}

\resetcounters

\bibliographystyle{asp2010}

\markboth{Author1, Author2, and Author3}{Author's Final Checklist}

%\begin{document}

\title{ASP Author Template}
\author{Sample~Author1,$^1$ Sample~Author2,$^2$ and Sample~Author3$^3$
\affil{$^1$Institution Full Address for Author1}
\affil{$^2$Institution Full Address for Author2}
\affil{$^3$Institution Full Address for Author3}}

\begin{abstract}
This is the Astronomical Society of the Pacific (ASP) 2010 author template file.  This sample author template includes the ASP author checklist.
\end{abstract}

\section{The Template}
To fill in this template, make sure that you read and follow the ASPCS Instructions for Authors and Editors available for download online.  Hints and tips for including graphics, tables, citations, and other formatting helps are available there.

\subsection{The Author Checklist}
The following checklist should be followed when writing a submission to a conference proceedings to be published by the ASP.

\begin{itemize}
\checklistitemize
\item Article is within page limitations set by editor. 
\item Paper compiles properly without errors or warnings.
\item No fundamental modifications to the basic template are present, including special definitions, special macros, packages, \verb"\vspace" commands, font adjustments, etc. %(§ 3.3, p. 10)
\item Commented-out text has been removed. %(§ 3.3, p. 10,11)
\item Author and shortened title running heads are proper for the paper and shortened so page number is within the margin. %(§ 3.1, p. 4)
\item Paper checked for general questions of format and style, including, but not limited to, the following:
\begin{itemize}
  \item capitalization, layout, and length of running heads, titles  and \\sections/subsections;  % (§ 3.1, p. 4) (§ 3.2, p. 5) (§ 3.3, p. 8)
  \item page numbers within margin; % (§ 3.1, p. 4)
  \item author names spelled correctly and full postal addresses given; % (§ 3.2, p. 5-6)
  \item abstracts; % (§ 3.2, p. 7);
  \item all margins---left, right, top and bottom; % (§3.1, p. 4; §3.2, p. 5; §3.3, p. 9; §3.6, p. 21);
  \item standard font size and no Type 3 fonts; %(§ 3.3, pp. 10-11; § 3.6, p. 23; § 4.2, p. 25);
  \item spacing; % (§ 3.3, pp. 9-10);
  \item section headings. % (§ 3.3; p. 8).
\end{itemize}
\item All tables are correctly positioned within margins, are properly formatted, and are referred to in the text.  %(§ 3.5, pp. 16-20)
\item All figures are correctly positioned within margins, are minimum 300 dpi resolution, not too dark or too light, do not contain embedded fonts, and are referred to in the text.  All labeling or text will be legible with 10\% reduction.  Questionable images printed, checked and replaced if necessary.  Figures do not cover text or running heads, and proper permissions have been granted and acknowledged.  %(§ 3.6, pp. 21-24)
\item All acknowledgments and discussions are in proper format.  % (pp. 11-12, p. 20)
\item If there are acknowledgments at the end of the article, ensure that the author has used
the \verb"\acknowledgments" command and not the commands
\\ \verb"\begin{Acknowledgments}", \verb"\end{Acknowledgments}".
Acknowledgments should only be used for thanking institutions,
groups, and individuals who have directly contributed to the work.
\item All references quoted in the text are listed in the bibliography; all items in the bibliography have been referred to in the text.  % (§ 4, pp. 24-28)
\item All bibliography entries are in the proper format, using one of the referencing styles given. Each of the references is bibliographically complete, including full names of authors, editors, publishers, place of publication, page numbers, years, etc. % (§§ 4.2-4.3, pp. 25-28)
\item A complete Bib\TeX\ file is ready to submit to the editor.
\item References to preprints replaced with publication information when possible.
\end{itemize}

\acknowledgements The ASP would like to the thank the dedicated researchers that are publishing with the ASP.

\bibliography{editor}

%\end{document}


==> editor/backmatter/backmatter.tex <==
% This is the backmatter.tex LaTeX file -- ASP Conference Proceedings backmatter.
% Copyright 2010, Astronomical Society of the Pacific Conference Series
%\documentclass[11pt,twoside]{book}
%\usepackage{../asp2010}

%\begin{document}

\pagestyle{empty}
\null
\setlength{\headheight}{0cm}
\setlength{\headsep}{0cm}
\setlength{\textheight}{21.6cm}
\setlength{\footskip}{0cm}

\begin{center}
{\LARGE \bfseries {ASTRONOMICAL SOCIETY OF THE PACIFIC}\\}
\vspace{1.0cm}
\end{center}

\changelinespacing{1.2}

{\fontfamily{phv}\selectfont 

\begin{wrapfigure}{l}{5.0truecm}
  \vspace{-0.75cm}
  \centering
  \includegraphics[width=5.0truecm, trim=0 15 0 0]{./frontmatter/logo_bw.eps}
\end{wrapfigure}

\noindent 
\textsc{The Astronomical Society of the Pacific} is an international, 
nonprofit, scientific, and \,\,educational organization. 
Some 120 years ago, on a chilly February evening in San Francisco, 
astronomers from Lick Observatory and members of the Pacific Coast 
Amateur Photographic Association---fresh from viewing the New Year's Day 
total solar eclipse of 1889 a little to the north of the city---met to share 
pictures and experiences. Edward Holden, Lick's first director, complimented 
the amateurs on their service to science and proposed to continue the good 
fellowship through the founding of a Society ``to advance the Science of 
Astronomy, and to diffuse information concerning it.'' The Astronomical 
Society of the Pacific (ASP) was born.

\vspace{5pt}
The ASP's purpose is to increase the understanding and appreciation of 
astronomy by engaging scientists, educators, enthusiasts, and the public to 
advance science and science literacy. The ASP has become the largest 
general astronomy society in the world, with members from over 70 nations.

\vspace{5pt}
The ASP's professional astronomer members are a key component of the
Society. Their desire to share with the public the rich rewards of 
their work permits the ASP to act as a bridge, explaining the mysteries 
of the universe. For these members, the ASP publishes the Publications 
of the Astronomical Society of the Pacific (PASP), a well-respected monthly 
scientific journal. In 1988, Dr. Harold McNamara, the PASP editor at 
the time, founded the ASP Conference Series at Brigham Young University.  
The ASP Conference Series shares recent developments in 
astronomy and astrophysics with the professional astronomy community.

\bigskip

\begin{center}
{\Large To learn how to join the ASP or to make a donation, please visit \url{http://www.astrosociety.org}.}
\end{center}}

\vfill
\eject

% Second page, list of Monographs
\begin{center}
{\Large ASTRONOMICAL SOCIETY OF THE PACIFIC}\\
\vspace{5pt}
{\LARGE \bfseries MONOGRAPH SERIES}\\
\vspace{5pt}
{\small Published by the Astronomical Society of the Pacific}\\
\vspace{5pt}
The ASP Monograph series was established in 1995 to publish select
reference titles. For electronic versions of ASP Monographs, please see
\url{http://www.aspmonographs.org}.
%\end{center}

\noindent\hrulefill
\vspace{1.0em}

%\begin{center}
{\bf INFRARED ATLAS OF THE ARCTURUS SPECTRUM, 0.9-5.3$\mu$m}\\
eds. Kenneth Hinkle, Lloyd Wallace, and William Livingston (1995)\\
ISBN: 1-886733-04-X, e-book ISBN: 978-1-58381-687-5

\vspace{5pt}
{\bf VISIBLE AND NEAR INFRARED ATLAS \\ OF THE ARCTURUS SPECTRUM 3727-9300\AA}\\
eds. Kenneth Hinkle, Lloyd Wallace, Jeff Valenti, and Dianne Harmer (2000)\\
ISBN: 1-58381-037-4, e-book ISBN: 978-1-58381-688-2

\vspace{5pt}
{\bf ULTRAVIOLET ATLAS OF THE ARCTURUS SPECTRUM 1150-3800\AA}\\
eds. Kenneth Hinkle, Lloyd Wallace, Jeff Valenti, and Thomas Ayres (2005)\\
ISBN: 1-58381-204-0, e-book ISBN: 978-1-58381-689-9

\vspace{5pt}
{\bf HANDBOOK OF STAR FORMING REGIONS: VOLUME I\\
THE NORTHERN SKY}\\
ed. Bo Reipurth (2008)\\
ISBN: 978-1-58381-670-7, e-book ISBN: 978-1-58381-677-6

\vspace{5pt}
{\bf HANDBOOK OF STAR FORMING REGIONS: VOLUME II\\ 
THE SOUTHERN SKY}\\
ed. Bo Reipurth (2008)\\
ISBN: 978-1-58381-671-4, e-book ISBN: 978-1-58381-678-3
%\end{center}

%\begin{center}
\hrulefill
\vspace{5pt}

A complete list and electronic versions of ASPCS volumes
may be found at \url{http://www.aspbooks.org}.
\vspace{5pt}

All book orders or inquiries concerning the ASP Conference Series, 
ASP Monographs, or International Astronomical Union Volumes published 
by the ASP should be directed to:\\
\vspace{5pt}
Astronomical Society of the Pacific\\
390 Ashton Avenue\\
San Francisco, CA  94112-1722  USA\\
Phone: 800-335-2624 (within the USA)\\
Phone: 415-337-2126\\
Fax: 415-337-5205\\
Email: \url{service@astrosociety.org}
\vspace{10pt}

For a complete list of ASP publications, please visit
\url{http://www.astrosociety.org}.

\end{center}

%\end{document}


==> editor/bibtextest/bibtextest.tex <==
% This is the bibtextest.tex LaTeX file
% Copyright 2010, Astronomical Society of the Pacific Conference Series
% The purpose of this file is to test the BibTeX files.

%\documentclass[11pt,twoside]{article}
%\usepackage{../asp2010}

% This file, the should be in the directory where you will run BibTeX from, 
% not necessarily the directory this file (bibtextest.tex) is in.
\bibliographystyle{asp2010}  

\markboth{Bib\TeX\ Test}{Bib\TeX\ Test}

%\begin{document}

\title{Test for Your Bib\TeX\ File}

\begin{abstract}
This is a \LaTeXe\ file designed to test the Bib\TeX\ files.
\end{abstract}

\section*{Testing Bib\TeX\ }
Compile this file to test the Bib\TeX files created for this book.  You must run \LaTeXe\ on this file at least once, then run Bib\TeX\, from the base directory of the main \texttt{.bib} file, then run \LaTeXe\ at least once more.

\nocite{*}

% This file should be in the directory where you will run BibTeX from, 
% not necessarily the directory this file (bibtextest.tex) is in.
\bibliography{editor}

%\end{document}


==> editor/editor_checklist/editor_checklist.tex <==
% This is the aspauthor2010.tex LaTeX file
% Copyright 2010, Astronomical Society of the Pacific Conference Series

%\documentclass[11pt,twoside]{article}
%\usepackage{../asp2010}

\resetcounters

\bibliographystyle{asp2010}

\markboth{Editor's Final Checklist}{Editor's Final Checklist}

%\begin{document}
\label{editorchecklist}

\title{Editor's Final Checklist}

%\labelitemi{$\box$}

\section*{General}

\begin{itemize}
\checklistitemize
\item All articles received. If the contribution  is incomplete (missing files, etc.), or doesn't compile properly, ask the author
for whatever is missing or to correct the submission.  Review the articles and contact the author concerning any recommended changes.% (' 2.2)
\item All articles refereed, if applicable. % (' 1)
\item All articles edited for grammar, style and scientific content. % (' 2.3)
\item All articles included and compiled into a single volume that compiles without errors or warnings. % (' 3)
\item Each individual paper, all front matter, and the indexes appear in the compiled volume.
\item Pre-submission form sent to the editorial assistant (aspcs@aspbooks.org) when within two weeks of suspected submission.
\end{itemize}

\section*{Front Matter}

\begin{itemize}
\checklistitemize
\item Pages i to iv include all necessary information and are correct. % (' 5).
\item Front cover illustration has been designated, uploaded to the server, and appropriately acknowledged on page i % (' 5.3)
\item Dedication checked.  % (on p. v, if included)  (' 3.6; Chicago Manual of Style, 15th Ed. [Chicago], 1.36-37).
\item Table of contents checked for the following: % (p. v or p. vii if Dedication included) (' 3.6; Chicago 1.40): 
\begin{itemize}
\item proper spacing;
\item consistent style of author names (full names or initials/surname) not broken up by any line breaks;
\item appropriate line breaks---titles/authors do not run into column for page number;
\item no hyphenation in titles;
\item appropriate page breaks---part titles appear with at least one paper;
\item all front matter and back matter listed on correct page;
\item each title matches the paper title exactly;
\item all authors listed on table of contents and spelling of names match each paper.
\end{itemize}
\item All pagination of front matter is correct and matches the table of contents. % (' 3.6; Chicago 1.101)
\item Conference Photo is as large as possible, but within margins; photo key is included, if desired.  Photo appears on odd-numbered (right) page if single page layout.  If key or separate page caption is included, photo appears on even-numbered (left) page with caption/key on the following page. %(' 3.6)
\item One or two blank pages appear between front matter and main matter.
\end{itemize}

\section*{Main Matter}

\begin{itemize}
\checklistitemize
\item Each paper and entire volume checked for general questions of format and style, including, but not limited to, the following:
\begin{itemize}
  \item slugs; % (' 2.4); 
  \item capitalization and layout of running heads, titles, and sections/subsections;  % (' 2.4) (' 2.5)
  \item author names and addresses; % (' 2.4);
  \item abstracts; % (Author's Instructions, ' 3.2);
  \item margins---left, right, top and bottom; % ('' 2.2. 2.4, 2.7, 3.5, 3.6);
  \item font; % (' 3.4; Author's Instructions, '' 3.3, 3.6, 4.2);
  \item spacing; % (Author's Instructions, ' 3.3);
  \item session or part headings; % ('3.2).
\end{itemize}
\item Author and shortened title running heads are correct for the paper. % (' 2.4)
\item All page numbers are correct, in sequence, and within margins; no page numbers appear on session heading pages and blank pages. % (' 3.1).
\item All tables are correctly positioned within margins, are properly formatted, and are referred to in the text.  % (' 2.7, Author=s Instructions ' 3.5)
\item All figures are correctly positioned within margins, are minimum 300 dpi resolution, not too dark or too light, do not contain embedded fonts, and are referred to in the text.  All labeling or text will be legible with 10\% reduction.  Questionable images printed, checked and replaced if necessary.  Figures do not cover text or running heads, and proper permissions have been granted and acknowledged.  %(' 2.7, Author=s Instructions ' 3.6)
\item All acknowledgments and discussions are in the proper format.  % ('2.8) (' 2.10)
\item All references quoted in the text are listed in the bibliography; all items in the bibliography have been referred to in the text. The Bib\TeX\ file is complete by containing all references referred to in the volume.  % (' 2.9)
\end{itemize}

\section*{Back Matter}

\begin{itemize}
\checklistitemize
\item All indexes appear at the end of the volume.  Page references for items in indexes have been checked and are correct (if changes have been made to volume, indexes may need to be recompiled). % ('' 4 and 6.1)
\end{itemize}

\section*{Submission}
Submission at the ASPCS is defined by the entire volume compiling without errors or warnings on the ASPCS server, and that the book is considered ready to print.  ASPCS personnel must be notified that the book has been submitted.

\begin{itemize}
\checklistitemize
\item Zipped files uploaded to the ASPCS server at the URL provided by ASPCS.  %at http://aspcs linux.byu.edu/upload/. (' 7; online editor=s information, Step 3, Section 3.2)
\item Mailing list form (names, up-to-date street addresses, telephone numbers and email addresses for all recipients of printed book) e-mailed to aspcs@byu.edu. % (' 7; online editor=s information, Step
\item Volume compiled on the ASPCS server; each page checked for any problems or errors.  All necessary changes have been made to files on ASPCS server.  % (Online editor=s information, Step 3, Section 3.2)
\item ASPCS notified that the book is prepared for submission and ready for aesthetic review.
\end{itemize}

\bibliography{manual2010}

%\end{document}


==> editor/frontmatter/conf_photo.tex <==
\vspace{-1cm}
\booklandscapephoto{image file name}{Image caption.}


==> editor/frontmatter/copyrightpage.tex <==
% This is the copyrightpage.tex LaTeX file
% Copyright 2009, Astronomical Society of the Pacific Conference Series
% Do not modify this file!
% To make this file appear correctly make sure that the following is in the style file (asp2009.sty)
%    The Library of Congress LCCN number (supplied by ASP)
%    The ISBN (supplied by ASP)
%    The year of copyright assignment (which may not be the year of publication)
\null
\setlength{\headheight}{0cm}
\setlength{\headsep}{0cm}
\setlength{\textheight}{8.3in}
\setlength{\footskip}{0cm}
\pagestyle{empty}
\vfill
{\footnotesize
\begin{center}
ASTRONOMICAL SOCIETY OF THE PACIFIC\\
\smallskip
390 Ashton Avenue\\
San Francisco, California, 94112-1722, USA\\
\medskip
Phone: 415-337-1100\\
Fax: 415-337-5205\\
E-mail: \url{service@astrosociety.org}\\
Web site: \url{www.astrosociety.org}\\
E-books: \url{www.aspbooks.org}\\
\bigskip
First Edition\\
\raisebox{1.5pt}{\tiny\copyright}\hspace{2pt}\cpryear\ by Astronomical Society of the Pacific\\
ASP Conference Series\\
All rights reserved.\\
\medskip
\end{center}
No part of the material protected by this copyright notice may be
reproduced or utilized in any form or by any means---graphic,
electronic, or mechanical, including photocopying, taping,
recording, or by any information storage and retrieval
system---without written permission from the Astronomical Society of the Pacific.\\
\bigskip
\begin{center}
ISBN:~\ISBN \\
e-book ISBN:~\eISBN \\
\bigskip
Library of Congress (LOC) Cataloging in Publication (CIP) Data:\\
Main entry under title\\
Library of Congress Control Number (LCCN):~\LCCN \\
\end{center}
\begin{center}
Printed in the United States of America by Sheridan Books, Ann Arbor, Michigan.

This book is printed on acid-free paper.
\end{center}
}


==> editor/frontmatter/cover.tex <==
% This is the cover.tex LaTeX file -- Not needed in a typical book submission.
% Copyright 2009, Astronomical Society of the Pacific Conference Series
\null
\setlength{\headheight}{0cm}
\setlength{\headsep}{0cm}
\setlength{\textheight}{21.6cm}
\setlength{\footskip}{0cm}
\pagestyle{empty}

\vfill
\begin{figure}[!h]
\plotfiddle{frontmatter/book_logo.eps}{0truecm}{0}{120}{120}{-126}{-20}
\end{figure}

\begin{center}

\hrulefill\\
{\LARGE \bfseries
\bigskip
VOLUME~\volume\\
\bigskip
}
\end{center}

\begin{center}
{\LARGE \bfseries ASP CONFERENCE SERIES\\
{\Large INSTRUCTIONS FOR AUTHORS AND
EDITORS\\}}
\end{center}
\vfill

\bookfigure{frontmatter/tryst.eps}{}

\begin{center}
{\Large
Edited by\\
\vspace{0.05in}
T.~J.~Mahoney, Lisa~B.~Roper, and Jonathan~Barnes
}
\end{center}

\pagebreak

\bookblankpage


==> editor/frontmatter/dedication.tex <==
\markboth{Dedication}{Dedication}
\pagestyle{myheadings}
\title{}
\thispagestyle{plain}
\null
\vfill
\begin{center}
{\Large\bfseries Dedication}
\smallskip
%\begin{figure}[!h]
%\end{figure}
%\plotone{}
\end{center}
\smallskip
\noindent {\small 
% INSERT TEXT OF DEDICATION HERE.
}
\vfill\eject


==> editor/frontmatter/foreword.tex <==
% This is the foreword.tex LaTeX file -- Please change only the indicated parts.
% Copyright 2009, Astronomical Society of the Pacific Conference Series
\markboth{Foreword}{Foreword}
\pagestyle{myheadings}
\thispagestyle{plain}
\section*{\Large\bfseries Foreword}
\bigskip
\parindent=2em

%%% FOREWORD -- Place the foreword text here
\noindent
Forward text goes here.

\bigskip

\noindent
Author

\noindent Author's Title



==> editor/frontmatter/halftitle.tex <==
% This is the halftitle.tex LaTeX file -- Please change only the indicated parts.
% Copyright 2009, Astronomical Society of the Pacific Conference Series
\null
\setlength{\headheight}{0cm}
\setlength{\headsep}{0cm}
\setlength{\textheight}{21.6cm}
\setlength{\footskip}{0cm}
\pagestyle{empty}
\begin{center}
{\large \bfseries \halftitle{}\\}
\end{center}
\vfill

\providecoverinfo

\pagebreak


==> editor/frontmatter/halftitle_verso.tex <==
% This is the halftitle_verso.tex LaTeX file
% Copyright 2009, Astronomical Society of the Pacific Conference Series
% Do not modify this file!
\null
\setlength{\headheight}{0cm}
\setlength{\headsep}{0cm}
\setlength{\textheight}{21.6cm}
\setlength{\footskip}{0cm}
\pagestyle{empty}
\begin{center}
{\large{ASTRONOMICAL SOCIETY OF THE PACIFIC\\
\vspace{3pt}
CONFERENCE SERIES}}\\
\end{center}
\begin{center}
{\scshape a series of books on recent developments in astronomy and astrophysics}\\
\medskip
{\bfseries
\hrulefill\\
{Volume~\volume\\}
\vspace{-0.22truecm}
\hrulefill
}
\end{center}
\vfill

\aspeditorialstaff

\bigskip

\aspaddress

\vfill

\asppubcommittee

\vfill
\vspace{0.1in}
\begin{center}
{\small

ASPCS volumes may be found online with color images at \url{http://www.aspbooks.org}.\\
ASP Monographs may be found online at \url{http://www.aspmonographs.org}.\\ \hfill\\
\vspace{.1in}
For a complete list of ASPCS Volumes, ASP Monographs, and\\
other ASP publications see
\url{http://www.astrosociety.org/pubs.html}}.\\ \hfill\\
\vspace{0.1in}
All book order and subscription inquiries should be directed to the ASP at 
800-335-2626 (toll-free within the USA) or 415-337-2126,\\ 
or email \url{service@astrosociety.org}
\end{center}
\eject\pagebreak


==> editor/frontmatter/participants.tex <==
% This is the participants.tex LaTeX file -- ASP Conference Proceedings style attendee list.
% Copyright 2010, Astronomical Society of the Pacific Conference Series
\markboth{Participants}{Participants}
\pagestyle{myheadings}

% Format information for each attendee according to \attendee macro.
%
%    \attendee{NAME}{EMAIL}{AFFIL}{ADDRESS}

\makeatletter
\makeatother

{
\parindent 0pt
\parskip .8ex
\columnsep .6in

\thispagestyle{plain}
\section*{\Large\bfseries Participants}
\thispagestyle{plain}
%%\raggedright
\begin{flushleft}
\input{frontmatter/participants.att}
\end{flushleft}
\parindent 2em
}
% Uncomment the following if needed to remove running head on the blank page following the participants list.
%\bookblankpage


==> editor/frontmatter/preface.tex <==
% This is the preface.tex LaTeX file
% Copyright 2009, Astronomical Society of the Pacific Conference Series
\markboth{Preface}{Preface}
\pagestyle{myheadings}
\thispagestyle{plain}
\aindex{Mahoney, T. J.}
\aindex{Roper, Lisa B.}
\section*{\Large\bfseries Preface}
\bigskip
\parindent=2em

\noindent 
Preface text goes here.

\bigskip

\noindent Preface Author
\vfill\eject
\thispagestyle{empty}


==> editor/frontmatter/titlepage.tex <==
% This is the titlepage.tex LaTeX file
% Copyright 2009, Astronomical Society of the Pacific Conference Series
% Only modify sections as noted!
\pagestyle{empty}
\null
\setlength{\headheight}{0cm}
\setlength{\headsep}{0cm}
\setlength{\textheight}{21.6cm}
\setlength{\footskip}{0cm}
\pagestyle{empty}
\begin{center}
{\large{ASTRONOMICAL SOCIETY OF THE PACIFIC\\
\vspace{3pt}
CONFERENCE SERIES}}\\
\end{center}
\begin{center}
\medskip
{\bfseries \hrulefill\\
{Volume~\volume\\
}
\vspace{-0.28truecm}
\hrulefill
}
\end{center}
\vspace{1.1truecm}
\begin{center}
{\Large \bfseries \maintitle{}\\}
\end{center}

\providemeetinginfo

\bigskip
\begin{center}
{Edited by}\\
\end{center}

\provideeditorone

\provideeditortwo

\provideeditorthree

\provideeditorfour

\provideeditorfive

\vfill
\begin{figure}[!h]
\plotfiddle{frontmatter/logo_bw.eps}{3.2truecm}{0}{30}{30}{-53}{-15}
\end{figure}

\begin{center}
{\small
SAN FRANCISCO}
\end{center}

\pagebreak

